When eBPF Meets Machine Learning: On-the-fly OS Kernel Compartmentalization

Compartmentalization effectively prevents initial corruption from turning into a successful attack. This paper presents O2C, a pioneering system designed to enforce OS kernel compartmentalization on the fly. It not only provides immediate remediation for sudden threats but also maintains consistent system availability through the enforcement process. O2C is empowered by the newest advancements of the eBPF ecosystem which allows to instrument eBPF programs that perform enforcement actions into the kernel at runtime. O2C takes the lead in embedding a machine learning model into eBPF programs, addressing unique challenges in on-the-fly compartmentalization. Our comprehensive evaluation shows that O2C effectively confines damage within the compartment. Further, we validate that decision tree is optimally suited for O2C owing to its advantages in processing tabular data, its explainable nature, and its compliance with the eBPF ecosystem. Last but not least, O2C is lightweight, showing negligible overhead and excellent sacalability system-wide.

==> sections/relatedwork.tex <==
\section{Related Work}





\noindent\textbf{Other Kernel Hardening.}
\yc{can be removed}
Various strategies have been developed to mitigate the risks associated with security incidents.
Kernel patches~\cite{zhang2021investigation,shariffdeen2021automated,tian2012identifying, kernelApplyingPatches} and live patches~\cite{arnold2009ksplice, chen2017adaptive} offer direct solutions by fixing kernel vulnerabilities to prevent corruption.
Linux kernel protections~\cite{kernsecKernelSelf} include structure randomization~\cite{lwnRandomizingStructure}, metadata protection~\cite{lwnSLUBFreelist,SlubImprove}, and Kernel Address Space Layout Randomization (KASLR)\cite{lwnFunctionGranular}.
Additional measures like AutoSlab\cite{grsecurityGrsecurityAUTOSLAB} and PAX\_USERCOPY~\cite{lwnHardenedUsercopy} have been developed by PaX/Grsecurity~\cite{grsecurityGrsecurity}.
Academic research has also proposed the use of reference monitors to enforce specific protection policies, such as CFI and DFI.
Notable works in this area include XPFO~\cite{kemerlis2014ret2dir}, RedLeaf~\cite{narayanan2020redleaf}, VirtualGhost~\cite{criswell2014virtual}, KCoFI~\cite{criswell2014kcofi}, NestedKernel~\cite{dautenhahn2015nested}, $\mu$Scope~\cite{uscope21}, MemSentry~\cite{koning2017no}, xMP~\cite{proskurin2020xmp}, and Kasper~\cite{DBLP:conf/ndss/JohannesmeyerKR22}.
Kernel debloating techniques, such as FACE-CHANGE~\cite{gu2014face}, KASR~\cite{zhang2018kasr}, and SHARD~\cite{abubakar2021shard}, aim to reduce the kernel's attack surface by limiting the code accessible to user applications.
In contrast to these approaches, \sys focuses on isolating vulnerable portions of modules from the kernel while maintaining the integrity of code, data, control flow, and APIs within the compartment.

